User-Friendly Customized Generation with Multi-Modal Prompts

Text-to-image generation models have seen considerable advancement, catering to the increasing interest in personalized image creation. Current customization techniques often necessitate users to provide multiple images (typically 3-5) for each customized object, along with the classification of these objects and descriptive textual prompts for scenes. This paper questions whether the process can be made more user-friendly and the customization more intricate. We propose a method where users need only provide images along with text for each customization topic, and necessitates only a single image per visual concept. We introduce the concept of a ``multi-modal prompt'', a novel integration of text and images tailored to each customization concept, which simplifies user interaction and facilitates precise customization of both objects and scenes. Our proposed paradigm for customized text-to-image generation surpasses existing finetune-based methods in user-friendliness and the ability to customize complex objects with user-friendly inputs. Our code is available at $\href{https://github.com/zhongzero/Multi-Modal-Prompt}{https://github.com/zhongzero/Multi-Modal-Prompt}$.

==> 5-future-work.tex <==
\section{Future Work}

The paradigm we proposed is supported for the situation of multiple images in the multi-modal prompt, but due to the limitation of current stable diffusions, the performance for multiple images situation doesn't achieve a good level. The specific reason is discussed in the supplementary material. Future work will try to use more advanced diffusion models, such SDXL \cite{SDXL}, to test the performance of our paradigm for multiple images situation, and also find some tricks to improve the performance. Another thing is that in our definition of multi-modal prompt, we restrict some conditions, such as the users want to customize the main objects in the images. Future work can focus on the more general definition of multi-modal prmopt, which means we will need to understand the meaning of the multi-modal prompt from the whole, and analysis the semantic information of both the image part and the text part.

